Just Roll with It: Exploring the Mitigating Effects of Postural Alignment on Vection-Induced Cybersickness in Virtual Reality Over Time

Cybersickness remains a significant challenge in virtual reality (VR), limiting its usability across various applications. Existing mitigation strategies focus on optimising VR hardware and/or software and enhancing self-motion perception to minimise sensory conflict. However, anticipatory postural adaptation, a strategy widely studied with regards to motion sickness while being driven, has not been systematically examined in VR. Therefore, in this study, we explore whether adopting comfort-orientated postural movements, based on the literature, mitigates cybersickness. We conducted an exploratory analysis using a cumulative link mixed model (CLMM) on secondary data from a VR-based postural alignment experiment. Results indicate that misalignment between trunk roll and the virtual trajectory increases the odds of reporting higher cybersickness scores by 5%. Additionally, each additional minute in VR increases the odds of reporting higher cybersickness scores (FMS scores) by 11% %, but prolonged exposure leads to a 75% % reduction in the odds of reporting cybersickness symptoms, suggesting adaptation effects. Individual differences also play a role, with higher cybersickness susceptibility increasing the odds of reporting higher symptom severity by 8%. These findings indicate that anticipatory postural adaptation could serve as a natural mitigation strategy for cybersickness. VR applications, particularly in training and simulation, may benefit from designing adaptive cues that encourage users to align their posture with virtual movement. Future research should explore real-time postural feedback mechanisms to enhance user comfort and reduce cybersickness.

==> OldResults.tex <==

separate models were created to investigate RMSE trunk roll alignment and time in minutes on self-reported FMS scores. Thus, our models are defined as:

\begin{equation} \label{Equation1}
    \text{FMS Scores}_i \sim \text{RMSE\_TrunkRoll}_i + \text{VIMSSQ}_i + \text{Group}_i + (1 | \text{ID}_i)\
\end{equation}

\begin{equation} \label{Equation2}
    \text{FMS Scores}_i \sim \text{Minutes}_i * \text{Route}_i + \text{Group}_i + \text{VIMSSQ}_i + (1 | \text{ID}_i)
\end{equation}

\begin{equation} \label{Equation3}
    \text{FMS Scores}_i \sim \text{Minutes}_i * \text{Route Section}_i + \text{Group}_i + \text{VIMSSQ}_i + (1 | \text{ID}_i)
\end{equation}

In Equation 1, we are only interested in RMSE trunk roll angles and include group and visually induced motion sickness susceptibility (Total VIMSSQ Scores) as covariate variables. To evaluate time in minutes, we first compare the pre-and post-condition routes separately in Equation 2 because they had the same time duration, in which we have the same covariates as Equation 1 with the addition of ``route". Then, in Equation 3, we investigate the condition route by itself and replace the covariate of ``route" with ``route section" since the 23 minutes contained numerous structured breaks, resulting in four sections. Finally, since Participant 9 is missing some data, we conducted two variants of the CLMM models, one with the data from Participant 9 and another excluding Participant 9 altogether. 

%-------------------------------- results --------------------------------------------------
\section{Results}
Below, we report our statistically significant results. Since our two variants of CLMM for each model offer the same significance with and without Participant 9 in the analysis, we choose to report the version with some of the data from Participant 9. You can find the results of all statistical analyses in our supplementary material. 

%----------------------- RMSE Trunk Roll Alignment ----------------------
\subsection{Trunk Roll Alignment and the Relationship on FMS Scores}
To investigate the relationship between trunk roll alignment with the angles of the routes in MATE-AV (RMSE Trunk Roll) on self-reported motion sickness (FMS scores), we conducted a CLMM (Equation 1).
The random intercept for participants had a variance of 3.541 (SD = 1.882), indicating a high variability amongst participants regarding their baseline scores. The results suggest that RMSE for trunk troll alignment is a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = 0.047, SE = 0.020, z = 2.402, p = .016). Suggesting that for each unit increase on the log-odds scale regarding RMSE trunk roll values (decrease in trunk roll alignment with the angles of a virtual route), the odds of self-reporting a higher motion sickness score (FMS) increase approximately by 5\% (Odds ratio = 1.05), suggesting a gentle increase as a predictor variable. 

For the two covariates in this CLMM, the results suggest that motion sickness susceptibility (Total VIMSSQ scores) is a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = 0.074, SE = 0.029, z = 2.556, p = .011). Suggesting that for each unit increase in motion susceptibility scores (Total VIMSSQ scores), the odds of self-reporting a higher motion sickness score (FMS) increase approximately by 8\% (Odds ratio = 1.08), suggesting another gentle increase as a predictor variable. However, the covariate for the participant's group (Control or VR-Training) is not a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = -0.934, SE = 1.067, z = -0.875, p = .382). The threshold coefficients between the ordinal categories from this CLMM can be found in table \ref{tab:CLMM_RMSE}.

\begin{table} [!h]
    \caption{Threshold coefficients for the CLMM model: FMS Scores and RMSE Trunk Roll Angles}
    \centering
    \begin{tabular}{|l|r|r|r|}
        \hline
        Threshold Coefficient & Estimate $\beta$ & SE & z\\
        \hline
         $0|1$ & 1.352 & 1.333 & 1.014\\
         $1|2$ & 3.195 & 1.337 & 2.389\\
         $2|3$ & 4.815 & 1.349 & 3.569\\
         $3|4$ & 6.388 & 1.363 & 4.687\\
         $4|5$ & 7.566 & 1.379 & 5.485\\
         $5|6$ & 8.705 & 1.411 & 6.171\\
         $6|7$ & 9.156 & 1.432 & 6.394\\
         $7|8$ & 10.317 & 1.546 & 6.672\\
        \hline
    \end{tabular}
    \label{tab:CLMM_RMSE}
\end{table}

%---------------------- Time and FMS Scores -------------------------------
\subsection{Time and the Relationship on FMS Scores}
To investigate the relationship between time in minutes and self-reported motion sickness (FMS scores), we conducted two CLMMs (Equations 2 and 3).

\subsubsection{Pre-Condition and Post-Condition Routes}
First, we analyse time in minutes based on the shorter routes used for the pre-condition and post-condition routes (Equation 2). For this analysis, we only conduct the variant with Participant 9 since there is no corresponding missing data for the pre-condition and post-condition routes.
The random intercept for participants in the shorter routes had a variance of 3.192 (SD = 1.787), indicating a high variability amongst participants regarding their baseline scores. The results suggest that time in minutes is a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = 0.290, SE = 0.080, z = 3.625, p = \textless.001). Suggesting that for each additional minute spent in VR, the odds of self-reporting a higher motion sickness score (FMS) increase approximately by 34\% (Odds ratio = 1.33). Route was not a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = -0.185, SE = 0.606, z = -0.306, p = .760), and nor was there a statistically significant interaction effect for route and minutes spent in VR ($\beta$ = -0.043, SE = 0.115, z = -0.373, p = .709).

Similar to our previous CLMM, motion sickness susceptibility (Total VIMSSQ scores) was again a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = 0.083, SE = 0.028, z = 2.942, p = .003). Suggesting that for each unit increase in motion susceptibility scores (Total VIMSSQ scores), the odds of self-reporting a higher motion sickness score (FMS) increase approximately by 9\% (Odds ratio = 1.09). However, the participant's group (Control or VR-training) is not a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = -0.916, SE = 1.037, z = -0.883, p = .377). The threshold coefficients between the ordinal categories from this CLMM can be found in table \ref{tab:CLMM_TimeShort}.

\begin{table} [!h]
    \caption{Threshold coefficients for the CLMM model: FMS Scores and Time in the Shorter Route (Pre- and Post-condition routes)}
    \centering
    \begin{tabular}{|l|r|r|r|}
        \hline
        Threshold Coefficient & Estimate $\beta$ & SE & z\\
        \hline
         $0|1$ & 2.572 & 1.352 & 1.902\\
         $1|2$ & 4.240 & 1.371 & 3.092\\
         $2|3$ & 5.826 & 1.408 & 4.137\\
         $3|4$ & 7.452 & 1.447 & 5.151\\
         $4|5$ & 8.673 & 1.478 & 5.869\\
         $5|6$ & 9.351 & 1.507 & 6.206\\
         $6|7$ & 9.748 & 1.530 & 6.371\\
         $7|8$ & 10.790 & 1.636 & 6.596\\
        \hline
    \end{tabular}
    \label{tab:CLMM_TimeShort}
\end{table}

%------------------ Condition route, time and FMS -----------------------
\subsubsection{Condition Route}
%Note that this is the only time we get a difference for excluding participant 9. Suddenly, there's an interaction effect. The effect of minutes decreases with more condition routes, decreasing the probability of reporting higher motion sickness.
Lastly, we analyse time in minutes based on the longer route used for the condition route (Equation 3).
The random intercept for participants in the condition route had a variance of 4.66 (SD = 2.159), indicating a high variability amongst participants regarding their baseline scores. The results suggest that time in minutes is again a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = 0.263, SE = 0.091, z = 2.893, p = .004). Suggesting that for each additional minute spent in VR, the odds of self-reporting a higher motion sickness score (FMS) increase approximately by 30\% (Odds ratio = 1.30). The section of the condition route (sections in between breaks) was not a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = 0.037, SE = 0.398, z = 0.092, p = .926), nor was there an interaction effect exists for the section of the condition route (sections in-between breaks) and minutes spent in VR on self-reported motion sickness (FMS scores) ($\beta$ = -0.037, SE = 0.020, z = -1.895, p = .058).

Similar to our other CLMMs, motion sickness susceptibility (Total VIMSSQ scores) was again a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = 0.080, SE = 0.034, z = 2.358, p = .018). Suggesting that for each unit increase in motion susceptibility scores (Total VIMSSQ scores), the odds of self-reporting a higher motion sickness score (FMS) increase approximately by 8\% (Odds ratio = 1.08). However, again, the participant's group (Control or VR-training) is not a statistically significant predictor of self-reported motion sickness (FMS scores) ($\beta$ = -1.162, SE = 1.186, z = -0.979, p = .327). The threshold coefficients between the ordinal categories from this CLMM can be found in table \ref{tab:CLMM_TimeCondition}.

\begin{table} [!h]
    \caption{Threshold coefficients for the CLMM model: FMS Scores and Time in the Condition Route}
    \centering
    \begin{tabular}{|l|r|r|r|}
        \hline
        Threshold Coefficient & Estimate $\beta$ & SE & z\\
        \hline
         $0|1$ & 2.789 & 1.680 & 1.660\\
         $1|2$ & 5.068 & 1.699 & 2.983\\
         $2|3$ & 6.960 & 1.727 & 4.031\\
         $3|4$ & 8.731 & 1.758 & 4.968\\
         $4|5$ & 9.910 & 1.787 & 5.544\\
         $5|6$ & 11.928 & 1.918 & 6.221\\
         $6|7$ & 12.655 & 2.046 & 6.184\\
        \hline
    \end{tabular}
    \label{tab:CLMM_TimeCondition}
\end{table}


